Simple Ingredients for Offline Reinforcement Learning

Offline reinforcement learning algorithms have proven effective on datasets highly connected to the target downstream task. Yet, leveraging a novel testbed (MOOD) in which trajectories come from heterogeneous sources, we show that existing methods struggle with diverse data: their performance considerably deteriorates as data collected for related but different tasks is simply added to the offline buffer. In light of this finding, we conduct a large empirical study where we formulate and test several hypotheses to explain this failure. Surprisingly, we find that scale, more than algorithmic considerations, is the key factor influencing performance. We show that simple methods like AWAC and IQL with increased network size overcome the paradoxical failure modes from the inclusion of additional data in MOOD, and notably outperform prior state-of-the-art algorithms on the canonical D4RL benchmark.

==> sections/d4rl_antmaze_values_10cri.tex <==
\begin{tabular}{lcccccccccccccccc}
    \toprule
     & \multicolumn{16}{c}{mean/sem} \\
     agent & \multicolumn{2}{c}{IQL} & \multicolumn{2}{c}{ASAC} & \multicolumn{2}{c}{AWAC} & \multicolumn{2}{c}{TD3} & \multicolumn{2}{c}{TD3+BC} \\
    actor dim & \multicolumn{4}{c}{1024} & \multicolumn{4}{c}{1024} & \multicolumn{4}{c}{1024} & \multicolumn{4}{c}{1024} \\
    num cri & \multicolumn{4}{c}{10} & \multicolumn{4}{c}{10} & \multicolumn{4}{c}{10} & \multicolumn{4}{c}{10} \\
    critic num layers & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{3} \\
    actor num layers & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{5} \\
    critic model & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} \\
    actor model & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} \\
    score processing & \multicolumn{2}{c}{softmax} & \multicolumn{2}{c}{softmax} & \multicolumn{2}{c}{asac buffer} & \multicolumn{2}{c}{asac buffer} & \multicolumn{2}{c}{softmax} & \multicolumn{2}{c}{softmax} & \multicolumn{2}{c}{none} & \multicolumn{2}{c}{none} \\
    num es & 1 & 50 & 1 & 50 & 1 & 50 & 1 & 50 & 1 & 50 & 1 & 50 & 1 & 50 & 1 & 50 \\
    task &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
    \midrule
     antmaze-large-diverse-v0 & 40.8 / 1.3 & 61.7 / 1.3 & 57.4 / 1.6 & 63.4 / 1.7 & 42.8 / 3.6 & 50.9 / 1.2 & 12.0 / 1.0 & 52.4 / 3.0 & 44.3 / 1.3 & 52.4 / 3.3 & 34.8 / 7.2 & 44.8 / 6.7 & 11.2 / 1.7 & 6.5 / 3.7 & 2.8 / 2.4 & 4.4 / 2.3 \\
     antmaze-large-play-v0 & 40.1 / 1.2 & 51.4 / 1.6 & 27.3 / 1.3 & 13.8 / 2.1 & 36.1 / 1.9 & 43.3 / 1.4 & 8.1 / 0.3 & 12.6 / 1.7 & 31.4 / 1.6 & 39.9 / 1.1 & 14.1 / 7.1 & 12.5 / 1.1 & 0.8 / 0.5 & 0.0 / 0.0 & 0.7 / 0.3 & 0.0 / 0.0 \\
     antmaze-medium-diverse-v0 & 74.9 / 1.5 & 83.1 / 0.7 & 78.3 / 1.3 & 80.2 / 1.9 & 77.1 / 2.0 & 83.3 / 1.3 & 65.6 / 1.6 & 88.7 / 0.6 & 79.2 / 0.7 & 84.7 / 0.6 & 83.7 / 1.4 & 87.1 / 0.9 & 38.4 / 15.7 & 27.3 / 16.7 & 12.4 / 0.6 & 17.3 / 1.3 \\
     antmaze-medium-play-v0 & 65.8 / 4.5 & 81.4 / 1.3 & 77.0 / 1.0 & 86.6 / 1.2 & 77.7 / 1.4 & 83.6 / 1.4 & 59.2 / 1.4 & 87.2 / 1.4 & 79.3 / 1.2 & 86.2 / 0.8 & 67.0 / 6.1 & 85.2 / 0.7 & 68.2 / 1.6 & 68.0 / 1.4 & 16.5 / 0.9 & 9.2 / 9.2 \\
     antmaze-umaze-diverse-v0 & 71.6 / 2.1 & 82.3 / 0.7 & 84.3 / 2.1 & 87.5 / 0.6 & 63.5 / 5.6 & 75.5 / 1.7 & 77.9 / 6.7 & 79.3 / 1.7 & 86.7 / 1.0 & 74.4 / 2.8 & 39.4 / 15.0 & 39.6 / 15.7 & 83.5 / 5.9 & 64.1 / 17.5 & 53.3 / 14.8 & 40.9 / 10.3 \\
     antmaze-umaze-v0 & 87.3 / 0.6 & 96.2 / 0.3 & 93.2 / 1.3 & 95.8 / 1.0 & 94.8 / 0.6 & 98.8 / 0.2 & 88.7 / 0.4 & 98.6 / 0.4 & 97.8 / 0.1 & 98.7 / 0.3 & 91.1 / 0.4 & 98.9 / 0.2 & 96.8 / 0.3 & 99.3 / 0.1 & 97.6 / 0.4 & 99.2 / 0.3 \\
    total & 380.4 & 456.1 & 417.5 & 427.3 & 391.9 & 435.4 & 311.4 & 418.9 & 418.7 & 436.1 & 330.2 & 368.0 & 299.0 & 265.1 & 183.4 & 170.9 \\
    \bottomrule
    \end{tabular}
    

==> sections/d4rl_antmaze_values_5cri.tex <==
\begin{tabular}{lcccccccccccccccc}
    \toprule
     & \multicolumn{16}{c}{mean/sem} \\
     agent & \multicolumn{2}{c}{IQL} & \multicolumn{2}{c}{ASAC} & \multicolumn{2}{c}{AWAC} & \multicolumn{2}{c}{TD3} & \multicolumn{2}{c}{TD3+BC} \\
    actor dim & \multicolumn{4}{c}{1024} & \multicolumn{4}{c}{1024} & \multicolumn{4}{c}{1024} & \multicolumn{4}{c}{1024} \\
    num cri & \multicolumn{4}{c}{5} & \multicolumn{4}{c}{5} & \multicolumn{4}{c}{5} & \multicolumn{4}{c}{5} \\
    critic num layers & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{3} \\
    actor num layers & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{5} & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{5} \\
    critic model & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} \\
    actor model & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} & \multicolumn{2}{c}{modern} & \multicolumn{2}{c}{simple} \\
    score processing & \multicolumn{2}{c}{softmax} & \multicolumn{2}{c}{softmax} & \multicolumn{2}{c}{asac buffer} & \multicolumn{2}{c}{asac buffer} & \multicolumn{2}{c}{softmax} & \multicolumn{2}{c}{softmax} & \multicolumn{2}{c}{none} & \multicolumn{2}{c}{none} \\
    num es & 1 & 50 & 1 & 50 & 1 & 50 & 1 & 50 & 1 & 50 & 1 & 50 & 1 & 50 & 1 & 50 \\
    task &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
    \midrule
     antmaze-large-diverse-v0 & 42.1 / 1.7 & 60.4 / 1.2 & 59.8 / 3.2 & 64.4 / 1.3 & 40.0 / 1.6 & 49.9 / 1.5 & 10.3 / 1.4 & 49.2 / 0.8 & 43.0 / 2.2 & 43.0 / 3.4 & 16.9 / 10.6 & 32.0 / 1.1 & 18.8 / 1.5 & 9.9 / 9.9 & 7.2 / 3.9 & 8.7 / 1.3 \\
     antmaze-large-play-v0 & 38.9 / 1.7 & 54.2 / 1.1 & 26.2 / 2.3 & 22.6 / 3.7 & 33.4 / 2.4 & 43.8 / 2.4 & 4.7 / 2.2 & 12.3 / 1.0 & 32.0 / 1.8 & 42.2 / 0.8 & 7.2 / 4.6 & 17.3 / 0.7 & 7.2 / 4.3 & 8.3 / 5.4 & 0.6 / 0.6 & 5.6 / 3.5 \\
     antmaze-medium-diverse-v0 & 73.2 / 1.4 & 82.9 / 1.1 & 77.0 / 2.0 & 85.6 / 0.6 & 78.3 / 1.1 & 82.3 / 0.8 & 63.8 / 1.6 & 89.1 / 1.5 & 77.0 / 0.6 & 83.2 / 1.5 & 48.0 / 19.6 & 85.8 / 1.1 & 65.7 / 2.5 & 75.0 / 7.5 & 17.7 / 7.2 & 61.9 / 14.1 \\
     antmaze-medium-play-v0 & 71.0 / 1.5 & 82.9 / 0.7 & 78.5 / 1.9 & 86.5 / 0.7 & 74.1 / 1.3 & 84.9 / 1.4 & 51.5 / 4.4 & 86.7 / 1.2 & 77.0 / 1.4 & 85.6 / 1.7 & 63.3 / 15.9 & 84.6 / 1.0 & 70.5 / 1.7 & 52.4 / 17.6 & 15.7 / 11.1 & 24.2 / 10.0 \\
     antmaze-umaze-diverse-v0 & 77.3 / 3.5 & 86.6 / 0.7 & 82.3 / 3.6 & 83.9 / 0.9 & 65.7 / 3.3 & 81.1 / 2.9 & 71.1 / 2.2 & 72.1 / 1.5 & 62.5 / 2.6 & 72.8 / 3.3 & 48.5 / 10.3 & 42.0 / 17.8 & 67.7 / 7.8 & 71.7 / 4.9 & 69.4 / 3.7 & 68.1 / 5.4 \\
     antmaze-umaze-v0 & 88.6 / 1.0 & 96.1 / 0.7 & 91.0 / 0.7 & 96.6 / 0.4 & 95.2 / 0.8 & 98.7 / 0.1 & 91.2 / 2.1 & 99.0 / 0.2 & 96.9 / 0.7 & 97.8 / 0.5 & 89.8 / 1.4 & 98.2 / 0.3 & 74.6 / 18.6 & 94.1 / 1.2 & 89.7 / 4.1 & 96.0 / 1.2 \\
    total & 391.1 & 463.1 & 414.8 & 439.6 & 386.7 & 440.8 & 292.6 & 408.5 & 388.3 & 424.8 & 273.7 & 359.8 & 304.3 & 311.5 & 200.3 & 264.6 \\
    \bottomrule
    \end{tabular}
    
